A Temporal Modeling Framework for Video Pre-Training on Video Instance Segmentation

Contemporary Video Instance Segmentation (VIS) methods typically adhere to a pre-train then fine-tune regime, where a segmentation model trained on images is fine-tuned on videos. However, the lack of temporal knowledge in the pre-trained model introduces a domain gap which may adversely affect the VIS performance. To effectively bridge this gap, we present a novel video pre-training approach to enhance VIS models, especially for videos with intricate instance relationships. Our crucial innovation focuses on reducing disparities between the pre-training and fine-tuning stages. Specifically, we first introduce consistent pseudo-video augmentations to create diverse pseudo-video samples for pre-training while maintaining the instance consistency across frames. Then, we incorporate a multi-scale temporal module to enhance the model's ability to model temporal relations through self- and cross-attention at short- and long-term temporal spans. Our approach does not set constraints on model architecture and can integrate seamlessly with various VIS methods. Experiment results on commonly adopted VIS benchmarks show that our method consistently outperforms state-of-the-art methods. Our approach achieves a notable 4.0% increase in average precision on the challenging OVIS dataset.

==> tex/fig_num_of_training.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/num_of_training_inference.pdf}
    \caption{The both figures depict the performance with varying frame counts during pre-training in the training and inference stages. The optimal performance is achieved when the training and inference phases generate a three-frame pseudo-video.\QZ{the left figure is number of training pseudo-frames, the right is inference pseudo-frames, both training and inference on COCO benchmark. The purpose of this figure is to illustrate that when training and inference maintain the same pseudo-video length, the best performance is achieved on the COCO benchmark. And even if using only a image for inference, the performance will not drop too much.}}
    
    \label{fig:image_group}
 \end{figure*}

==> tex/fig_sotaplot.tex <==
\begin{figure}

    \centering
    \includegraphics[width=0.5\columnwidth]{figures/teaser.pdf}
    
    \caption{Comparison with the previous state-of-the-art (SOTA) method on major video instance segmentation (VIS) benchmarks. With ResNet-50 as the backbone, our approach achieved notable enhancements of 0.9\%, 3.3\%, and 4.0\% in AP on YouTubeVIS-2019 \cite{vis}, YouTubeVIS-2021 \cite{vis2021}, and OVIS \cite{ovis}, respectively. The compelling performance gain effectively mitigates the gap between pre-training and fine-tuning.}
    \label{fig:perf}
\end{figure} 

==> tex/fig_teaser.tex <==
\begin{figure*}[t]
    \centering

    \subfigure[Previous Image Pre-training VIS]{\label{subfig:image}
    \begin{overpic}[width=0.47\textwidth]{figures/imagepretrain.pdf}
    \put(12,48.5){\scriptsize Image}
    \put(12,22.5){\scriptsize Video}
    \put(47,3){\tiny \rotatebox{90}{Temporal}}
    \put(51,6){\tiny \rotatebox{90}{Model}}
    \put(41,24){\tiny Init}
    \put(47,32.5){\tiny \rotatebox{90}{Image}}
    \put(51,32.5){\tiny \rotatebox{90}{Model}}
    \end{overpic}
    }
    \subfigure[Our Video Pre-training VIS]{\label{subfig:video}
    \begin{overpic}[width=0.47\textwidth]{figures/videopretrain.pdf}
    \put(4,49){\scriptsize Pseudo-Video}
    \put(12,22.5){\scriptsize Video}
    \put(47,3){\tiny \rotatebox{90}{Temporal}}
    \put(51,6){\tiny \rotatebox{90}{Model}}
    \put(41,24){\tiny Init}
    \put(47,30.5){\tiny \rotatebox{90}{Temporal}}
    \put(51,32.5){\tiny \rotatebox{90}{Model}}
    \end{overpic}
    }
    \caption{Pipelines of previous methods and our method. (a) Conventional VIS is where pre-trained image models are employed to initialise temporal models for video tasks. (b) Our approach involves the generation of pseudo-videos, which are then used to train specifically tailored temporal models. Subsequently, these trained models are utilised to initialise the temporal modules in video tasks.}
    \label{fig:teaser}
    \vspace{-8pt}
\end{figure*} 


==> tex/tab_allabl.tex <==
\begin{table}[t]
  \centering
  \begin{minipage}{0.5\linewidth}
    \caption{Ablation study on modules.}
    \label{tab:allabl}
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{ccccc}
    \toprule
    MSTM & CPVA & VP & AP$^{\mathtt{YV19}}$ & AP$^{\mathtt{OVIS}}$ \\
    \midrule
    - & - & - & 59.7 & 27.4 \\
    $\checkmark$ & - & - & 59.8 & 28.3 \\
    $\checkmark$ & $\checkmark$ & - & 60.2 & 28.5 \\
    $\checkmark$ & - & $\checkmark$ & 60.5 & 32.0 \\
    \rowcolor{gray!30}  
    $\checkmark$ & $\checkmark$ & $\checkmark$ & \textbf{61.8} & \textbf{32.6} \\
    \bottomrule
    \end{tabular}%
    }
  \end{minipage}
  \hfill
  \begin{minipage}{0.44\linewidth}
    \caption{Rotation angle settings.}
    \label{tab:rotation}
    \centering
    \begin{tabular}{lcc}
    \toprule
    Rotation & AP\textsuperscript{YV19} & AP\textsuperscript{OVIS} \\
    \midrule
    \rowcolor{gray!30}
    $\pm15^\circ$ & 59.7 & 27.4 \\
    $\pm45^\circ$ & 57.8 & 26.4 \\
    $\pm60^\circ$ & 58.8 & 27.2 \\
    \bottomrule
    \end{tabular}
  \end{minipage}
\end{table}


==> tex/tab_augabl.tex <==
\begin{table}
  \caption{Ablation on different augmentation techniques in the video pre-training phase. VMoSp: Video Morph \& Splice; CoSt: Consistent Stochastic Augmentation.}
  \label{tab:abl}
  \centering
    \begin{tabular}{ccccccc}
    \toprule
    Rotation & VMoSp & CoSt & AP &AP$_\text{s}$ &AP$_\text{m}$ &AP$_\text{l}$    \\
    \midrule
    $\checkmark$  & & & 44.7 & 24.7  & 48.3 & 64.9                     \\
    $\checkmark$&   $\checkmark$ & & 44.8 & 24.4  & 48.8 & 65.9                     \\
    $\checkmark$&  &$\checkmark$   & 45.0 & 25.3  & 48.7 &\textbf{66.5}  \\
    \rowcolor{gray!30}
    $\checkmark$& $\checkmark$ &$\checkmark$   & \textbf{45.3} & \textbf{25.4}  & \textbf{49.1} &66.2  \\
    \bottomrule
    \end{tabular}%
\end{table}

==> tex/tabs_cost.tex <==
\begin{table}[t]
  \centering
  \caption{Different augmentation methodS.}
  \begin{tabular}{lcc}
    \toprule
    Augmentations & AP\textsuperscript{YV19} & AP\textsuperscript{OVIS} \\
    \midrule
    N/A &  54.1 & 24.5 \\
    Rotation & 59.7 & 27.4 \\
    Copy \& Paste & 59.1 & 26.8 \\
    \rowcolor{gray!30}
    Crop Shift & 58.6 & 26.1 \\
    Autoaug & 59.5 & 26.8 \\
    \rowcolor{gray!30}
    CoSt & 60.0 & 27.4 \\
    VMoSp & 59.8 & 27.6 \\
    \bottomrule
  \end{tabular}
  \label{tab:augmentation}
\end{table}

